NTIRE 2026 Challenge on Robust AI-Generated Image Detection in the Wild

This paper presents an overview of the NTIRE 2026 Challenge on Robust AI-Generated Image Detection in the Wild, held in conjunction with the NTIRE workshop at CVPR 2026. The goal of this challenge was to develop detection models capable of distinguishing real images from generated ones in realistic scenarios: the images are often transformed (cropped, resized, compressed, blurred) for practical usage, and therefore, the detection models should be robust to such transformations. The challenge is based on a novel dataset consisting of 108,750 real and 185,750 AI-generated images from 42 generators comprising a large variety of open-source and closed-source models of various architectures, augmented with 36 image transformations. Methods were evaluated using ROC AUC on the full test set, including both transformed and untransformed images. A total of 511 participants registered, with 20 teams submitting valid final solutions. This report provides a comprehensive overview of the challenge, describes the proposed solutions, and can be used as a valuable reference for researchers and practitioners in increasing the robustness of the detection models to real-world transformations.

==> sec/3_solutions_short.tex <==
\section{Team and methods}

\subsection{MICV}\label{MICV}

% \subsubsection{Team details}\label{team-details}
% \begin{itemize}
% \item Team name: MICV
% \item Team leader name: Chuanbiao Song
% \item Team leader emails: songchuanbiao.scb@antgroup.com
% \item Affiliation: Ant Group
% \end{itemize}

\subsubsection{Technical Details}\label{technical-details}

% \paragraph{Overview}\label{overview}

In this work, we propose a robust ensemble-based framework for
% AI-generated image detection, specifically designed to address the
challenges of domain generalization and cross-platform detection. Our
approach centers on three core pillars:

% \begin{itemize}
% \item
%   Hierarchical Data Strategy: We curate a large-scale, multi-source
%   training corpus that integrates open-source academic benchmarks,
%   synthetic images from cutting-edge generative models, and
%   high-fidelity samples from closed-source commercial APIs, ensuring
%   comprehensive coverage of diverse generative artifacts.
% \item
%   Ensemble-based Architecture: We utilize the powerful representation
%   capabilities of multiple DINOv3 backbones, organized into two distinct
%   model committees. By employing a late-fusion strategy that averages
%   the detection probabilities derived from these ensembles, we achieve a
%   more holistic and discriminative signature of AI-generated content.
% \item 
%   Robust Augmentation: To enhance robustness against ``in-the-wild''
%   degradations, we implement a hierarchical, difficulty-aware data
%   augmentation pipeline. Combined with a Focal Loss-driven optimization
%   and Stochastic Weight Averaging (SWA), our approach effectively bridges
%   the distribution gap between laboratory benchmarks and real-world
%   unconstrained imagery.
% \end{itemize}


\paragraph{Data Collection}\label{data-collection}

High-quality, large-scale, and diverse datasets are fundamental to the
robustness and generalizability of AI-Generated Image detection. To
effectively emulate the complex, ``in-the-wild'' distribution of
generative artifacts, we curate a comprehensive training corpus
comprising millions of samples. Our data acquisition strategy is
hierarchical, categorized into four primary tiers:

\begin{itemize}
\item
  Open-Source Datasets: To establish a solid foundation for cross-domain
  generalization, we integrate a diverse array of open-source resources,
  ranging from established academic benchmarks to large-scale
  repositories hosted on platforms like HuggingFace. This collection
  includes, but is not limited to, GenImage, WildFake, AIGIBench,
  CommunityForensics, and So-Fake-Set, along with representative
  datasets sourced from open-source communities. By aggregating these
  heterogeneous data sources, we ensure that our model is exposed to a
  wide spectrum of generation paradigms and realworld artifacts,
  significantly enhancing the scalability and effectiveness of our
  model.
\item
  Open-Source Generative Models: To align with the rapid evolution of
  generative architectures, we construct a substantial synthetic dataset
  using state-of-the-art open-source models. Our pipeline encompasses a
  multifaceted range of generation tasks, including Text-to-Image (T2I),
  Image-to-Image (I2I), image editing and inpainting, leveraging
  representative models such as Qwen-Image, Z-Image, and the FLUX series
  to capture the distinct artifacts inherent in contemporary
  architectures.
\item
  Closed-Source Commercial Models: Given the prevalence of closedsource
  platforms in real-world applications, we supplement our corpus with
  high-fidelity samples obtained via official APIs. By integrating
  outputs from industry-leading engines such as Seedream, Kling,
  GPT-Image, and Nano-banana-pro, we effectively mitigate the
  distribution shift between open-source research models and proprietary
  commercial systems, thereby enhancing the detector's practical
  deployment efficacy.
\item
  Challenge-Specific Datasets: To further expand our set of training
  samples, we utilized the image samples provided by the competition
  organizers.
\end{itemize}

\paragraph{Methodology}\label{methodology}

As illustrated in Figure \hyperref[MICV_architecture]{1,} we propose a feature
fusion architecture for AIgenerated image detection. Our approach
leverages the powerful feature representation capabilities of DINOv3
backbones by employing two distinct subnetworks, each designed to
process image features through an ensemble of pretrained backbones.

Specifically, the architecture comprises two independent streams: the
first stream aggregates feature maps from a committee of four DINOv3
backbones, while the second stream integrates features from a separate
committee of two DINOv3 backbones. Within each sub-network, the
aggregated backbone features are processed through a dedicated
projection layer to map them into a latent space, followed by a
multi-layer perceptron (MLP) head that produces the detection
probability. To derive the final prediction, we average output probabilities from both streams.

To bridge the distribution shift between controlled benchmarks and
challenging ``in-the-wild'' imagery, we design a hierarchical,
stochastic data augmentation pipeline structured by difficulty levels.
Our pipeline progresses from simple, individual transformations to
complex combinatorial perturbations. While the former applies individual
degradations such as blur, noise, geometric shifts or compression, the
latter employs multi-stage pipelines that simulate complex degradations.
This hierarchical and multi-faceted augmentation strategy effectively
narrows the domain gap, ensuring superior detection performance even in
highly unconstrained and degraded environments.


\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{team_figures/MICV/_page_2_Figure_4.jpeg}
    \caption{MICV method scheme. DINOv3-based detection framework.}
    \label{MICV_architecture}
\end{figure}


% \paragraph{Implementation Details}\label{implementation-details}

% We initialize our framework using pretrained DINOv3 backbones and
% perform end-to-end fine-tuning. During training, images are randomly
% cropped and resized to 512 × 512 pixels, supplemented by our
% hierarchical augmentation pipeline. During inference, images are
% directly resized to 512 × 512 to preserve the global spatial context. The
% model is trained on 32 NVIDIA A100 GPUs for 10 epochs, with the entire
% procedure completing in approximately 8 hours.

% \begin{itemize}
% \item
%   Objective Function: We employ Focal Loss as our primary objective
%   function to address the potential imbalance in sample difficulty and
%   to mitigate the dominance of easy-negative samples. The focus
%  parameter $\gamma$ is set to 2.0, and the balance parameter $\alpha$ is
%   empirically set to 0.5, to ensure that the model focuses on hard-to-classify
%   generative artifacts.
% \item
%   Optimization Strategy: We utilize the AdamW optimizer with a weight
%   decay of 0.02. The learning rate is initialized at 1×10-5. To ensure
%   training stability, we implement a linear warmup strategy over the
%   first epoch, followed by a Cosine Annealing schedule to gradually
%   decay the learning rate for the remainder of the training process. We
%   employ Stochastic Weight Averaging (SWA) over the final epochs to
%   aggregate model weights. This refinement yields a more stable and
%   generalized weight configuration, which serves as our final inference
%   model.
% \item
%   Evaluation and Refinement: We evaluate model performance using the
%   Area Under the Receiver Operating Characteristic curve (ROC AUC) on a
%   dedicated validation set, which is curated by sampling 10,000
%   labelbalanced images from the official training corpus. To ensure a
%   robust assessment under challenging conditions, we apply a static
%   version of the hierarchical data augmentation pipeline to this
%   validation set to assess robustness.
% \end{itemize}

% \paragraph{Acknowledgments}\label{acknowledgments}

% We sincerely thank the open-source community, whose contributions have been instrumental to the development of this framework. We are especially grateful to the creators of various AIGC detection benchmarks for providing the foundation of our study, and to the research teams behind state-of-the-art generative models for open-sourcing the architectures and tools that enabled our high-quality data synthesis.

\subsection{Ant International}

% \subsubsection{Team Information}
% \textbf{Team:} Ant International \\
% \textbf{Authors:} Zhiqiang Yang, Yongwei Tang, Zhiqiang Wu, Jia Wen Seow, Hong Vin Koay, Haodong Ren, Feng Xu, Shuai Chen.

\subsubsection{Introduction}
The rapid progress of text-to-image (T2I) generation has made synthetic images increasingly photorealistic, creating a pressing need for robust AI-generated image detection.  
Our solution for the NTIRE 2026 Robust AI-Generated Image Detection Challenge is guided by three principles:
\begin{itemize}
    \item \textbf{Massive and diverse data:} large-scale multi-source training set with extensive augmentations.
    \item \textbf{Model scaling:} leveraging very large vision backbones for improved generalization.
    \item \textbf{Expert ensemble:} combining two complementary specialists trained with different strategies.
\end{itemize}

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{team_figures/Ant_International/method_architecture.pdf}
    \caption{Ant International method scheme.}
    \label{Ant_International_scheme}
\end{figure}

\subsubsection{Data Preparation and Augmentation}
Our training set contains approximately 1 million images from three sources:
\begin{itemize}
    \item Official NTIRE 2026 challenge training set.
    \item Self-generated synthetic images from \textit{LongCat-Image}, \textit{Z-Image}, \textit{Qwen-Image}, and \textit{Qwen-Image-2512}.
    \item Open-source detection datasets: \textit{Dragon} and \textit{UniGenBench}.
\end{itemize}

To improve robustness, we apply a four-level offline augmentation pipeline:
\begin{itemize}
    \item \textbf{Level 1 (Clean):} original images.
    \item \textbf{Level 2 (Mild):} 1--3 random distortions, severity sampled with mean 0 and std 2.5.
    \item \textbf{Level 3 (Moderate):} 3--6 random distortions, mean 2.5 and std 2.0.
    \item \textbf{Level 4 (Heavy):} fixed 6 distortions, mean 3.5, std 1.0.
\end{itemize}

\subsubsection{Backbone Selection}
We evaluated several large-scale vision backbones (\textit{eva02-large}, \textit{eva-giant}, \textit{siglip2-giant}, \textit{DINOv3-7B}).  
Experiments showed strong scaling behavior: larger models and higher input resolutions consistently improved performance and generalization.  
Therefore, we selected \textbf{DINOv3-7B} as the base architecture.

\subsubsection{Dual-Expert Ensemble Architecture}
Our final model is a dual-expert ensemble consisting of two independently fine-tuned \textbf{DINOv3-7B} models (total 14B parameters).  
Given an input image, both experts produce detection scores, which are aggregated into a final robust prediction.  
Both experts are trained with full-parameter fine-tuning on NVIDIA B200 GPUs.

\subsubsection{Expert Training Strategy}

\paragraph{Expert 1: High-Resolution Specialist}
\begin{itemize}
    \item \textbf{Data:} Levels 2, 3, and 4 only.
    \item \textbf{Pooling:} \texttt{attention\_pooling}.
    \item \textbf{Input resolution:} $512 \times 512$.
    \item \textbf{Online augmentation:} random horizontal flip ($p=0.5$) + AugMix (\texttt{m6-w3-d1}).
    \item \textbf{Training setup:} 1 epoch, learning rate $1\times 10^{-6}$, Model EMA, AMP, no dropout.
\end{itemize}

\paragraph{Expert 2: Robustness-Focused Specialist}
\begin{itemize}
    \item \textbf{Data:} Levels 1, 2, 3, and 4.
    \item \textbf{Pooling:} \texttt{first\_token\_pooling}.
    \item \textbf{Input resolution:} $288 \times 288$.
    \item \textbf{Training duration:} 10 epochs.
\end{itemize}

% \begin{table}[h]
% \centering
% \caption{Hyperparameters for Expert 2.}
% \begin{tabular}{ll}
% \hline
% \textbf{Parameter} & \textbf{Value} \\
% \hline
% Backbone & \texttt{vit\_7b\_patch16\_dinov3.lvd1689m} \\
% Input size & $288 \times 288$ \\
% RandomResizedCrop scale & $[0.3,\,1.0]$ \\
% AutoAugment & \texttt{augmix-m6-w3-d1} \\
% Random erasing & 0.2 (\texttt{pixel} mode) \\
% Color jitter prob. & 0.1 \\
% Grayscale prob. & 0.05 \\
% Gaussian blur prob. & 0.1 \\
% Optimizer & AdamW \\
% Learning rate & $1\times 10^{-5}$ \\
% Betas & $(0.9, 0.999)$ \\
% Epsilon & $1\times 10^{-8}$ \\
% Weight decay & 0.05 \\
% Scheduler & Cosine annealing \\
% Warmup epochs & 0 \\
% Batch size / GPU & 12 (24 total on 2 GPUs) \\
% Model EMA & Enabled \\
% AMP & Enabled \\
% Layer-wise LR decay & 0.9 \\
% Dropout & 0.15 \\
% DropPath & 0.15 \\
% Label smoothing & 0.05 \\
% \hline
% \end{tabular}
% \end{table}

\subsubsection{Inference}
Inference consists of two steps:
\begin{enumerate}
    \item \textbf{Test-time augmentation (TTA):} each expert predicts on multiple augmented variants of each test image.
    \item \textbf{Weighted ensembling:} TTA outputs are aggregated per expert, then combined via weighted averaging across experts.
\end{enumerate}
On a single NVIDIA A100 GPU, the full pipeline runs at approximately \textbf{2.21 images/s} with \textbf{78.25 GB} VRAM usage.

% \subsubsection{Conclusion}
% Our NTIRE 2026 solution shows that robust AI-generated image detection benefits strongly from:
% \begin{itemize}
%     \item model scaling (DINOv3-7B),
%     \item large and diverse augmented data,
%     \item and complementary dual-expert ensembling.
% \end{itemize}
% By combining a high-resolution specialist and a robustness-focused specialist, we achieve strong generalization under real-world image transformations.

\subsection{TeleAI-TeleGuard. TeleAI Strategy for Robust AI-Generated Image Detection in the Wild}
\label{subsec:teleai_strategy}


\subsubsection{Proposed Method}
\label{subsubsec:proposed_method}

We propose a LoRA-based Pairwise Training (LPT) strategy to achieve robust detection of AI-generated images (AIGI). As shown in Figure~\ref{fig:lpt_pipeline}, this strategy consists of three components: foundation-model fine-tuning, distortion simulation, and pairwise optimization.

In addition to the distortions provided by the organizer, after inspecting the validation set we introduce three extra distortion types---\emph{Speckle Noise}, \emph{Color Cast}, and \emph{Organic Moire}---which better match the target data distribution. We also increase distortion severity by setting the mean of the Gaussian distribution to 3.

The foundation model in LPT is EVA-CLIP~\cite{sun2023evaclip}. Following LoRA-style fine-tuning~\cite{hu2022lora}, we adapt the linear layers in the multi-head self-attention (MHSA) and feed-forward network (FFN) of each visual transformer block.

To improve robustness without degrading clean-sample performance, we adopt pairwise optimization by jointly feeding clean images and their corresponding distorted versions in each batch. Features extracted from distorted images are corrected by an additional feed-forward network. The overall training loss is:
\begin{equation}
\mathcal{L} =
\mathcal{L}_{CE}(\mathbf{x}, \mathbf{y})
+ \alpha \cdot \mathcal{L}_{KL}(\mathbf{x}, \hat{\mathbf{x}})
+ \beta \cdot \mathcal{L}_{MSE}(\mathbf{f}_{x}, \mathbf{f}'_{\hat{x}}),
\label{eq:lpt_loss}
\end{equation}
where $\mathbf{x}$, $\hat{\mathbf{x}}$, $\mathbf{f}_{x}$, and $\mathbf{f}'_{\hat{x}}$ denote clean samples, distorted samples, clean-sample features, and corrected distorted-sample features, respectively. $\mathcal{L}_{CE}$, $\mathcal{L}_{KL}$, and $\mathcal{L}_{MSE}$ are cross-entropy, KL divergence, and mean squared error losses. We set $\alpha=0.5$ and $\beta=0.25$.

Experiments are conducted on eight NVIDIA A800 GPUs for 5 epochs. We use AdamW~\cite{loshchilov2017decoupled} with an initial learning rate of $2\times10^{-4}$ and a cosine annealing scheduler~\cite{loshchilov2016sgdr}. To further improve generalization, we additionally include the So-Fake~\cite{huang2025sofake} and Chameleon~\cite{yan2024sanity} datasets during training.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{team_figures/TeleAI-TeleGuard/_page_0_Figure_10.jpeg}
    \caption{TeleAI-TeleGuard method scheme. \textbf{Pipeline of LPT.} To achieve robust detection, the framework includes distortion simulation, foundation-model fine-tuning, and pairwise optimization.}
    \label{fig:lpt_pipeline}
\end{figure}

\subsection{INTSIG}
\label{subsec:INTSIG}

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{team_figures/INTSIG/method_architecture.pdf}
    \caption{INTSIG method scheme.}
    \label{INTSIG_scheme}
\end{figure}

\subsubsection{Model Training Strategies}
\label{subsubsec:model_training_strategies}

\paragraph{Overview.}
We develop five complementary detectors in a staged pipeline. Model~1 is a full fine-tuning baseline on DINOv3-Huge. Model~2 continues training with expanded data. Model~3 further increases robustness with stronger distortion augmentation. Model~4 introduces a high-resolution branch ($448\times448$). Model~5 replaces the backbone with MetaCLIP2 Giant and applies partial fine-tuning. This design balances in-domain accuracy and OOD robustness.

\paragraph{Model 1: Baseline.}
Model~1 uses DINOv3-Huge with an MLP head:
\begin{equation}
1280 \rightarrow 256 \xrightarrow{\mathrm{ReLU}+\mathrm{Dropout}(0.1)} 2.
\end{equation}
We use AdamW (betas $(0.9,0.999)$) with separate parameter groups: backbone lr $=2\times10^{-5}$, weight decay $=0.05$; head lr $=5\times10^{-4}$, weight decay $=0.01$. The learning-rate schedule is 10\% warmup followed by cosine annealing, stepped per batch. Cross-entropy is used as the training objective, and class imbalance is handled by a distributed weighted sampler.  
Training data includes the official training set, SoFake-OOD, and RRDataset (10\% validation split). Inputs are preprocessed with random resized crop ($256\times256$, bicubic, scale $(0.08,1.0)$, ratio $(0.75,1.3333)$), random horizontal flip, and color jitter. Distortion augmentation is enabled with probability 0.5 (up to 3 distortions, 3 levels). Training runs for 20 epochs on 8$\times$H800 (DDP), with per-GPU batch size 16/8 (train/val).

\paragraph{Model 2: Incremental training with dataset expansion.}
Starting from Model~1, we reduce learning rates (backbone $5\times10^{-6}$, head $5\times10^{-5}$) and expand training data to: official set + SoFake-OOD + RRDataset + Chameleon + 50\% GenImage\_val + AIGIBench\_test. Other settings are unchanged.

\paragraph{Model 3: Incremental training with enhanced augmentation.}
Model~3 continues from Model~2 while increasing distortion intensity to 5 distortions and 5 levels (augmentation probability remains 0.5). Other settings are unchanged.

\paragraph{Model 4: High-resolution path.}
Model~4 uses $448\times448$ inputs to capture finer artifacts. AdamW is retained with 5\% warmup and cosine annealing. Learning rates are set to $5\times10^{-5}$ (backbone) and $1\times10^{-3}$ (head). Training data is the official set only, with a 1\% validation split. Preprocessing follows the same policy as Model~1 but at $448\times448$ resolution. Distortion augmentation uses probability 0.5, with up to 3 distortions and 5 levels.

\paragraph{Model 5: Backbone replacement.}
Model~5 adopts MetaCLIP2 Giant. We partially fine-tune all LayerNorm parameters and the full parameters of the last two layers. 
% The classifier is:
% \begin{align}
% &\text{MLP1: } 1664 \rightarrow 2048 \rightarrow 512, \nonumber\\
% &\text{MLP2: } 512 \rightarrow 256 \rightarrow 2.
% \end{align}
Training uses the official set, learning rate $10^{-4}$, and FocalLoss. Inputs are resized to $378\times378$; training includes random flip, random rotation, and random augmentation. Distortion augmentation is lighter (probability 0.2, 3 distortions, 3 levels).

% \begin{table}[t]
% \centering
% \small
% \setlength{\tabcolsep}{4pt}
% \renewcommand{\arraystretch}{1.1}
% \begin{tabular}{p{0.09\columnwidth}p{0.16\columnwidth}p{0.47\columnwidth}p{0.16\columnwidth}}
% \hline
% Model & Input & Core change & Weight \\
% \hline
% M1 & $256^2$ & DINOv3-Huge baseline & 0.3675 \\
% M2 & $256^2$ & Incremental data expansion & 0.0735 \\
% M3 & $256^2$ & Stronger distortion augmentation & 0.0490 \\
% M4 & $448^2$ & High-resolution branch & 0.2100 \\
% M5 & $378^2$ & MetaCLIP2 Giant backbone & 0.3000 \\
% \hline
% \end{tabular}
% \caption{Summary of training paths and ensemble weights.}
% \label{tab:model_paths}
% \end{table}

\subsubsection{Model Ensemble Strategy}
\label{subsubsec:ensemble_strategy}

\paragraph{Weighted hierarchical fusion.}
The final logit is computed as:
\begin{align}
\mathrm{Final\_Logit}
&= 0.7\Big[0.7(0.75M1 + 0.15M2 + 0.1M3) \nonumber\\
&\quad + 0.3M4\Big] + 0.3M5 .
\end{align}
Horizontal-flip TTA is applied to M3 and M4.

\paragraph{Dual-gating correction.}
We define directional confidence:
\begin{equation}
\mathrm{diff}=\mathrm{logit}_1-\mathrm{logit}_0.
\end{equation}
\textit{Gate-1 (strong consensus correction)} is triggered when M4 and M5 strongly agree ($|M4_{\mathrm{diff}}|\ge 8$, $|M5_{\mathrm{diff}}|\ge 3$), but the fused output has the opposite direction. We then shift the final logit by 2.5 toward the M4/M5 direction.  
\textit{Gate-2 (anomaly suppression)} is triggered when at least 3 models in $\{M1,M2,M3,M5\}$ agree while M4 disagrees; M4 is excluded and remaining weights are renormalized.

% \subsubsection{Engineering Optimization}
% \label{subsubsec:engineering_optimization}

% \paragraph{Parallel inference.}
% Inference runs with one CUDA stream per model, CPU-side multi-threaded preprocessing, and AMP for M1--M4.

% \paragraph{I/O and overlap.}
% We use asynchronous data loading (\texttt{num\_workers=4}) and prefetching (\texttt{prefetch=4}), overlapping CPU preprocessing with GPU inference to reduce idle time.

% \begin{table}[t]
% \centering
% \small
% \setlength{\tabcolsep}{4pt}
% \renewcommand{\arraystretch}{1.1}
% \begin{tabular}{p{0.24\columnwidth}p{0.37\columnwidth}p{0.31\columnwidth}}
% \hline
% Dimension & Technical solution & Effect \\
% \hline
% GPU parallelism & 5 independent CUDA streams & Full model overlap \\
% Compute precision & AMP for M1--M4 & $\sim$30\% throughput gain \\
% Data loading & Async I/O + prefetch=4 & Reduced wait time \\
% Pipeline & CPU/GPU overlap & Higher utilization \\
% \hline
% \end{tabular}
% \caption{Inference-time engineering optimizations.}
% \label{tab:eng_opt}
% \end{table}

\subsection{Vincentlc. Robust AI-Generated Image Detection via SigLIP2-Giant and Perturbation-Aware Training}
\label{sec:method_robust_siglip2}

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{team_figures/Vincentic/method_architecture.pdf}
    \caption{Vincentlc method scheme.}
    \label{Vincentic_architecture}
\end{figure}

\subsubsection{Overview}
We propose a simple yet effective framework for detecting AI-generated images in the wild.
Our method combines a pre-trained vision--language backbone with a lightweight linear classification head.
To improve robustness under severe real-world distribution shifts, we explicitly integrate the official image distortion pipeline used in challenging evaluation protocols~\cite{li2025bridging} into training, forcing the network to learn perturbation-invariant representations.

\subsubsection{Model Architecture}
\paragraph{Backbone Feature Extractor.}
We experimented with multiple scales of the SigLIP2 family and found that the largest variant, \texttt{siglip2-giant-opt-patch16-384}, achieves the strongest performance.
For downstream binary classification, we extract the patch-token sequence from the final hidden layer of the pre-trained SigLIP2 encoder~\cite{siglip2}.

\paragraph{Feature Aggregation and Classification Head.}
We evaluated several aggregation strategies, including CLS-token extraction, attention pooling, and multi-layer feature concatenation.
Empirically, global average pooling over all final-layer patch tokens yields the most robust and stable results.
The pooled feature vector is then fed into a single linear layer to produce real/fake logits.

\subsubsection{Robust Data Augmentation}
\paragraph{Spatial Transforms (``Squish'' Strategy).}
Instead of random resized cropping (which may remove localized forensic cues), we apply a ``squish'' strategy:
all images are directly resized to $384\times384$ (ignoring aspect ratio), followed by random horizontal flipping.
This preserves full image content while maintaining training efficiency.

\paragraph{Competition-Specific Distortions.}
We wrap the official \texttt{distort\_images} function into the PyTorch transform pipeline.
In our best run, we set \texttt{distortion\_prob=1.0}, so every training image is distorted, with up to three random post-processing operations sampled at multiple severity levels (\texttt{num\_levels=5}).
This aggressive augmentation acts as a strong regularizer and is a key driver of our Robust ROC AUC improvements.

% \subsubsection{Training Details}
% \paragraph{Optimization.}
% We train using Hugging Face Accelerate~\cite{accelerate} for distributed multi-GPU execution.
% Optimization uses AdamW~\cite{loshchilov2017decoupled} with batch size 24 per GPU.
% To preserve pre-trained backbone knowledge while adapting the classifier quickly, we use differential learning rates:
% $1\times10^{-5}$ for the SigLIP2 backbone and $3\times10^{-4}$ for the linear head.

% \paragraph{Learning Rate Schedule.}
% We apply cosine annealing with linear warmup (10\% of total steps) over 5 epochs, following SGDR-style scheduling~\cite{loshchilov2016sgdr}.

% \paragraph{Hardware and Acceleration.}
% Mixed-precision training is enabled to reduce memory footprint and improve throughput while maintaining numerical stability.

\subsection{Reagvis Labs. RAPID: Robust AI-Generated Prototype Image Detection}
\label{rapid-robust-ai-generated-prototype-image-detection}

We propose RAPID, a cascaded six-model ensemble for robust AI-generated image detection under realistic degradations. The system combines four complementary representation families: CLIP~\cite{radford2021clip}, SigLIP~\cite{zhai2023siglip}, SRM-style forensic residual modeling~\cite{fridrich2012rich}, and EVA-02 masked-image pretraining~\cite{fang2024eva02}. Each branch is fine-tuned with parameter-efficient adaptation (mainly LoRA~\cite{hu2022lora}), and final prediction is obtained by staged logit-space fusion. To keep memory low, models are executed sequentially; peak VRAM remains below 4\,GB.

\subsubsection{Architecture}
\label{architecture}

RAPID uses six detectors in a progressive refinement cascade. The main semantic branch (G4) is CLIP ViT-L/14 with LoRA on attention and MLP projections, followed by a GAPL prototype-attention head that compares normalized embeddings against learned forensic prototypes. A high-resolution SigLIP-v2 branch (384$\times$384) shares the same GAPL idea and improves sensitivity to fine local artifacts. In parallel, an SRM+Bayar ForensicCNN branch processes raw pixel inputs without normalization, explicitly modeling residual-domain inconsistencies. Two EVA-02 checkpoints provide complementary MIM-based cues: the original LoRA model and a retrained fixed-initialization variant with improved calibration under degradation. Finally, G4\_v2 (continued training from G4 EMA) performs last-step correction on difficult modern generations.

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{team_figures/Reagvis_Labs/method_architecture.pdf}
    \caption{Reagvis Labs method scheme. Overview of RAPID with staged logit fusion.}
    \label{fig:rapid_arch}
\end{figure}

\subsubsection{Logit-Space Cascade Fusion}
\label{score-fusion-4-stage-logit-blend}

All branches output probabilities in $[0,1]$. We combine them in logit space, where additive mixing is better calibrated than direct probability averaging.
\begin{equation}
\ell(p)=\log\frac{p}{1-p}.
\end{equation}

\begin{equation}
\begin{aligned}
s_{1a} &= \sigma\!\left(0.50L_{G4}+0.35L_{S}+0.15L_{R}\right),\\
b      &= \sigma\!\left(0.80L_{1a}+0.20L_{E}\right),\\
s_{2}  &= \sigma\!\left(0.85L_{b}+0.15L_{E_f}\right),\\
f      &= \sigma\!\left(0.89L_{2}+0.11L_{G4v2}\right).
\end{aligned}
\label{eq:rapid_fusion}
\end{equation}

\noindent
Here, $L_{G4}=\ell(G4)$, $L_S=\ell(\text{SigLIP})$, $L_R=\ell(\text{SRM})$, $L_E=\ell(\text{EVA02})$, $L_{E_f}=\ell(\text{EVA02}_{\text{fixed}})$, $L_{1a}=\ell(s_{1a})$, $L_b=\ell(b)$, $L_2=\ell(s_2)$, and $L_{G4v2}=\ell(G4_{\text{v2}})$.

This cascade was built incrementally through validation ablations; each stage was retained only if it improved robust AUC.

\subsubsection{Inference-Time Robustness}
\label{test-time-augmentation}

We apply 8-view TTA per model, mixing geometric and degradation-aware transforms (flip, multi-scale center crops, corner crops, blur, and JPEG perturbation). For sigmoid heads, we average logits across views and then apply sigmoid; for softmax heads, we average class probabilities. SigLIP uses resolution-matched 384px variants of the same views, while SRM uses bicubic resizing on raw $[0,1]$ inputs.

\subsubsection{Training Protocol}
\label{training-details}

All branches are trained on the official NTIRE 2026 data using AdamW with cosine decay and warmup, EMA checkpointing, and mixed precision where stable. Augmentations include random crop/flip, JPEG recompression, Gaussian blur/noise, and random resizing. Transformer branches use LoRA (typically $r=32$), while G4\_v2 is obtained by low-LR continuation from the G4 EMA checkpoint with SAM and CutMix for harder-sample generalization.

% \subsubsection{Runtime and Memory}
% \label{runtime-performance}

% Table~\ref{tab:rapid_runtime} reports per-model latency and memory on an H100.

% \begin{table}[t]
% \centering
% \setlength{\tabcolsep}{3.5pt}
% \renewcommand{\arraystretch}{1.05}
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{lccc}
% \toprule
% Model & Time (ms) & Peak VRAM (GB) & Fine-tuning \\
% \midrule
% G4 (CLIP+GAPL)       & $\sim$37 & 2.6 & LoRA $r{=}32$ (attn+MLP) \\
% SigLIP-v2            & $\sim$26 & 1.8 & LoRA $r{=}32$ (384px) \\
% SRM ForensicCNN      & $\sim$5  & 0.1 & full training (FP32) \\
% EVA-02 (original)    & $\sim$25 & 1.3 & LoRA $r{=}32$ + SwiGLU \\
% EVA-02 (fixed)       & $\sim$25 & 1.3 & LoRA $r{=}32$ retrain \\
% G4\_v2 (CLIP+GAPL)   & $\sim$37 & 2.6 & LoRA continuation \\
% \bottomrule
% \end{tabular}
% }
% \caption{Per-branch inference cost and memory. Sequential loading keeps total peak memory below 4\,GB.}
% \label{tab:rapid_runtime}
% \end{table}

\subsubsection{Design Rationale}
\label{key-design-decisions}

RAPID is built around complementarity: semantic and language-aligned features (CLIP/SigLIP), residual forensic cues (SRM), and MIM-driven representations (EVA-02) fail on different samples, making staged logit blending consistently stronger than any single branch. Prototype-attention heads improve interpretability by comparing each image to learned real/fake forensic anchors, while degradation-aware TTA stabilizes predictions under compression, blur, and scale shifts commonly observed in the wild.

\subsection{UESTC}

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{team_figures/UESTC/method_architecture.pdf}
    \caption{UESTC method scheme.}
    \label{UESTC_scheme}
\end{figure}

\paragraph{Overview.}
Our final detector is a multi-expert ensemble composed of four Vision Transformer backbones: two CLIP ViT-L/14 models~\cite{radford2021clip} and two SigLIP So400M Patch14-384 models~\cite{zhai2023siglip}.  
For each backbone, we attach a lightweight classification head that maps high-dimensional feature representations to binary predictions.  
Because the backbones have different native input configurations, we use backbone-specific preprocessing and standardize inputs to \(224\times224\) for CLIP and \(384\times384\) for SigLIP.  
Despite using four experts, inference remains efficient, with a peak GPU memory footprint of approximately 10\,GB.

\paragraph{Backbone selection.}
To identify suitable feature extractors, we conduct a large-scale empirical study over diverse backbones, including CLIP~\cite{radford2021clip}, SigLIP~\cite{zhai2023siglip}, MoCo~\cite{he2020moco}, Swin Transformer~\cite{liu2021swin}, ConvNeXt~\cite{liu2022convnext}, DINO~\cite{caron2021dino}, CoCa~\cite{yu2022coca}, and BEiT~\cite{bao2021beit}.  
We compare representation quality, computational efficiency, and robustness to synthetic artifacts.  
Empirically, CLIP and SigLIP provide the best trade-off between discriminative capability and cross-domain generalization, and therefore form the basis of the final system.

\paragraph{Data strategy.}
We improve robustness through two complementary components: training-set expansion and comprehensive degradation modeling.  
First, we expand the official training set with diverse synthesis pipelines, including state-of-the-art diffusion generators~\cite{ho2020ddpm,rombach2022high}, reconstruction pipelines, domain-transfer methods, and targeted adversarial attacks.  
This expansion introduces both realistic AI-generated samples and challenging hard negatives, exposing the detector to broader failure modes and emerging forgery artifacts.  
Second, we extend the official augmentation scripts with a wider array of degradation operators, covering complex blurs, noise patterns, compression artifacts, and advanced optical/digital distortions.  
These realistic perturbations encourage degradation-invariant representations and significantly improve robustness under distribution shifts caused by imaging conditions, transmission errors, and post-processing pipelines.

% \paragraph{Training paradigm.}
% We treat deepfake detection as more than a vanilla binary classification task and adopt a two-stage training strategy.  
% In Stage~1, each model is trained for two epochs with a standard binary objective (real vs.\ generated).  
% In Stage~2, we introduce feature-level self-distillation with dense supervision: intermediate feature maps from the epoch-2 checkpoint are used as dense targets, and the model is explicitly optimized to align current representations with these distilled features.  
% This dense alignment regularizes feature geometry, reduces overfitting to the competition distribution, and improves generalization to unseen generation methods and real-world domains.

% \paragraph{Inference.}
% At inference time, we average the predicted probabilities from four independently trained experts (two CLIP variants and two SigLIP variants) to produce the final robust prediction.

\subsection{PSU. PRISM: Paradigm-diverse Representation Integration for Synthesis-artifact Manifold Detection}
\label{subsec:prism}

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{team_figures/PSU/_page_1_Figure_0.jpeg}
    \caption{PSU method scheme.}
    \label{PSU_scheme}
\end{figure}

\subsubsection{Method Description}
\label{subsubsec:prism_method}

\textbf{PRISM} is a heterogeneous ensemble detector for AI-generated images, designed for robustness under JPEG compression, blur, noise, rescaling, and cropping. Our core hypothesis is that no single pre-training objective encodes the full forensic artifact manifold~\cite{wang2020cnn,corvi2023diffusiondetect}: contrastive objectives capture semantic inconsistencies; self-supervised patch objectives preserve texture discontinuities; supervised CNNs encode low-frequency spectral anomalies. Robust detection therefore requires \emph{explicit paradigm diversity}.

\paragraph{Prior work.}
Wang \textit{et al.}~\cite{wang2020cnn} showed CNN detectors generalize across GAN generators with augmentation, yet collapse under JPEG re-compression~\cite{gragnaniello2021critical}. Ojha \textit{et al.}~\cite{ojha2023towards} froze CLIP and trained a linear probe, achieving strong cross-generator generalization. PRISM extends this by (i) covering three paradigms beyond CLIP, (ii) paradigm-specific fine-tuning, and (iii) weighting by \emph{robust} AUC rather than clean accuracy.

\paragraph{Encoder pool.}
We instantiate $K{=}7$ encoders $\{\phi_k\}_{k=1}^K$ across three paradigms (Table~\ref{tab:prism_encoders}). For vision-language (VL) encoders (CLIP~\cite{radford2021clip}, SigLIP~\cite{zhai2023siglip}, EVA02~\cite{fang2024eva02}), features are $\ell_2$-normalized onto the unit hypersphere~\cite{wang2020alignmentuniformity}:
\[
\hat{z}_k = \frac{z_k}{\|z_k\|_2} \in \mathcal{S}^{d_k-1},
\]
preserving the contrastive geometry. DINOv2~\cite{oquab2023dinov2}, ConvNeXt~\cite{liu2022convnext}, and EfficientNet-V2~\cite{tan2021efficientnetv2} remain frozen; their features are passed directly to the classification head.

\paragraph{Paradigm-aware tuning.}
VL encoders undergo \emph{LayerNorm tuning}~\cite{wortsman2022robustfinetuning}: only LayerNorm scale/shift (about $0.03\%$ of weights) are updated, preventing catastrophic forgetting while adapting internal normalization to the forensic domain. All models use EMA ($\alpha{=}0.9995$) for checkpoint stabilization and calibrated posteriors. VL heads are two-layer MLPs ($h{=}512$); DINOv2 uses a linear probe. Training uses label-smoothed BCE ($\varepsilon{=}0.05$), AdamW ($\lambda{=}0.01$), cosine LR schedule, and fp16.

\begin{table}[t]
\centering
\small
\caption{PRISM encoder pool. $d$: feature dimension. LN: LayerNorm-only tuning. F: frozen encoder.}
\label{tab:prism_encoders}
\begin{tabular}{l l c c c}
\toprule
\textbf{Encoder} & \textbf{Paradigm} & \textbf{$d$} & \textbf{Tune} & \textbf{Head} \\
\midrule
CLIP ViT-L/14         & VL-Contrastive    & 1024 & LN & MLP-512 \\
SigLIP ViT-L/16       & VL-Contrastive    & 1024 & LN & MLP-512 \\
EVA02-Large           & VL-Contrastive    & 1024 & LN & MLP-512 \\
DINOv2 ViT-L/14       & Self-Supervised   & 1024 & F  & Linear \\
ConvNeXt-Large        & Supervised CNN    & 1536 & F  & MLP-512 \\
EfficientNet-V2-L     & Supervised CNN    & 1280 & F  & MLP-512 \\
CLIP ViT-B/16         & VL-Contrastive    & 512  & LN & MLP-256 \\
\bottomrule
\end{tabular}
\end{table}

\paragraph{Robust ensemble.}
Each model is scored on held-out validation data under all degradation types, yielding per-model robust AUC $A_k^{\mathrm{rob}}$. Normalized weights
\[
w_k = \frac{A_k^{\mathrm{rob}}}{\sum_j A_j^{\mathrm{rob}}}
\]
drive the ensemble. The final prediction with horizontal-flip TTA is
\begin{equation}
\hat{p} = \frac{1}{2}\left[\sum_k w_k\,p_k(x) + \sum_k w_k\,p_k(\mathcal{F}(x))\right].
\label{eq:prism_ensemble}
\end{equation}
Early stopping maximizes
\[
\mathcal{M} = 0.7A^{\text{rob}} + 0.3A^{\text{clean}}.
\]

\subsection{Shallow Real}

\subsubsection{Method Description}
\label{subsubsec:ntire2026_description}

As shown in Fig.~\ref{fig:ntire2026_pipeline}, we formulate robust AI-generated image detection as a binary classification task. Our model uses a DINOv3-Large backbone (following the DINO line of self-supervised visual encoders~\cite{oquab2023dinov2}), fine-tuned with Low-Rank Adaptation (LoRA)~\cite{hu2022lora} using rank $r=32$ and scaling factor $\alpha=64$.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{team_figures/Shallow_Real/_page_0_Figure_2.jpeg}
    \caption{Shallow Real method scheme. Overall pipeline of the proposed model.}
    \label{fig:ntire2026_pipeline}
\end{figure}

Final prediction is produced by a Multi-Aspect Classification (MAC) head operating on DINOv3 features. Specifically, the head aggregates:
(i) one \texttt{[CLS]} token,
(ii) four \texttt{[REG]} tokens, and
(iii) one \texttt{[AVG]} token computed as the average of the remaining patch tokens.
These six 1024-dimensional vectors are concatenated into a 6144-dimensional representation and passed to a two-layer MLP with an intermediate ReLU activation to output the binary score.

During training, we use three key techniques:
\begin{enumerate}
    \item \textbf{Dynamic resolution.}
    Input images are resized to random resolutions, where both height and width are sampled from $[384, 1152]$ (multiples of patch size 16), with a randomly selected interpolation method.

    \item \textbf{Deep supervision.}
    Auxiliary classification heads are attached to the last four layers of the DINOv3 backbone. Training loss is computed for each auxiliary output, while only the final-layer output is used at inference time. Each auxiliary head uses dropout with rate 0.2 in its fully connected layer.

    \item \textbf{Metric learning objective.}
    A supervised contrastive loss~\cite{khosla2020supcon} is added as an auxiliary objective alongside the primary binary cross-entropy loss, improving feature discrimination.
\end{enumerate}

The model is trained for 10 epochs using AdamW~\cite{loshchilov2017decoupled} with a linear learning-rate decay from $10^{-4}$ to $0$. Training uses the union of the official training set and the CommunityForensics dataset, with batch size 32 and the official data-augmentation pipeline.
